Colony-Enhanced Recurrent Neural Architecture Search: Collaborative Ant-Based Optimization

Crafting neural network architectures manually is a formidable challenge often leading to suboptimal and inefficient structures. The pursuit of the perfect neural configuration is a complex task, prompting the need for a metaheuristic approach such as Neural Architecture Search (NAS). Drawing inspiration from the ingenious mechanisms of nature, this paper introduces Collaborative Ant-based Neural Topology Search (CANTS-N), pushing the boundaries of NAS and Neural Evolution (NE). In this innovative approach, ant-inspired agents meticulously construct neural network structures, dynamically adapting within a dynamic environment, much like their natural counterparts. Guided by Particle Swarm Optimization (PSO), CANTS-N's colonies optimize architecture searches, achieving remarkable improvements in mean squared error (MSE) over established methods, including BP-free CANTS, BP CANTS, and ANTS. Scalable, adaptable, and forward-looking, CANTS-N has the potential to reshape the landscape of NAS and NE. This paper provides detailed insights into its methodology, results, and far-reaching implications.

==> sections/outlines.tex <==
\newpage
\section*{Outlines}

\begin{itemize}
    \item Why Multi-Colony?
    \item How Multi-Colony is a way of Active Inference?
    \item How Multi-Colony?
    \begin{itemize}
        \item PSO: different hyperparameters: evaporation-rate, mortality-rate, number-of-ants
        \item different parameters are dealt with as PSO positions
        
    \end{itemize}
    \item \textbf{CANTS}:
        \begin{itemize}
            \item 
        \end{itemize}
    
\end{itemize}

\subsection*{Thoughts about CANTS relation to Active Inference}
\begin{itemize}
    \item \textbf{Diversity and Specialization:} In nature, different ant colonies often specialize in specific tasks. For example, some colonies may focus on foraging for food, while others may prioritize defending the nest or caring for the brood. Similarly, your multiple colonies can be viewed as specialized teams, each with a specific focus within the NAS task. Some colonies might excel at exploring a wide range of network architectures, while others may be better at exploiting promising architectures. This diversity can help cover a broader part of the search space efficiently.
    \item  \textbf{Information Sharing:} Ants in different colonies may exchange information indirectly through various means like chemical trails or encounters at food sources. In your NAS approach, information sharing between colonies through PSO can be seen as a mechanism for indirect communication. The colonies can learn from each other's experiences and collectively improve their performance over time.
    \item \textbf{Parallel Exploration:} In nature, multiple ant colonies can simultaneously explore different regions of their environment. Similarly, your multi-colony NAS approach allows for parallel exploration of the neural architecture search space. This can lead to a more comprehensive exploration and a higher chance of discovering optimal architectures.
    \item \textbf{Competition and Cooperation:} Ant colonies often compete for resources, but they can also cooperate when facing common challenges. In your approach, while the colonies may compete to some extent, they ultimately cooperate through information sharing (PSO) to optimize the NAS process collectively. This balance between competition and cooperation can lead to a dynamic optimization process.
    \item \textbf{Adaptation and Learning:} Ant colonies exhibit adaptive behavior based on environmental conditions. In your NAS approach, each colony can adapt its exploration and exploitation strategies based on its own experiences and the shared information. This adaptability can help improve the overall performance of the optimization process.

\end{itemize}

% \input{sections/003.method_colonies_algo}


\begin{figure}
    \centering
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=.5\textwidth]{imgs/multi_col_schem.pdf}
        \caption{Subfigure 1}
        \label{fig:sub1}
  \end{subfigure}
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=.5\textwidth]{imgs/asynchronous.pdf}
        \caption{Subfigure 1}
        \label{fig:sub1}
  \end{subfigure}
\end{figure}

